Large Interferometer For Exoplanets (LIFE): III. Spectral resolution, wavelength range and sensitivity requirements based on atmospheric retrieval analyses of an exo-Earth

Temperate terrestrial exoplanets are likely common objects, but their discovery and characterization is very challenging. Concepts for optimized space missions to overcome these challenges are being studied. The LIFE initiative focuses on the development of a space-based mid-infrared (MIR) nulling interferometer probing the thermal emission of a large sample of exoplanets. We derive first estimates for the signal-to-noise (S/N), spectral resolution (R), and wavelength requirements for LIFE. Using an Earth-twin exoplanet as reference case, we quantify how well planetary/atmospheric properties can be constrained from MIR spectra of different quality. We simulate LIFE observations of an Earth-twin orbiting a G2V star at 10 pc from the Sun with different levels of exozodiacal dust emissions. We combine a cloud-free 1D radiative transfer model and the nested sampling algorithm to retrieve planetary/atmospheric properties from input spectra of different wavelength coverage, R, and S/N. We find that H2O, CO2, and O3 are detectable if S/N$\geq$10 (uncertainty $\leq\pm1.0$ dex). We find upper limits for N2O (abundance $\leq10^{-3}$). CO, N2, and O2 are unconstrained in all cases. The limit for a CH4 detection is R $= 50$, S/N $=10$. We further correctly determine the exoplanet radius (uncertainty $\leq\pm10\%$), surface temperature (uncertainty $\leq\pm20$K), and surface pressure (uncertainty $\leq\pm0.5$ dex). With the current LIFE design, the observation time required to reach the specified S/N amounts to $\sim7$ weeks with 4x2m apertures. We conclude that a minimum wavelength coverage of $4-18.5\mu$m, a R of 50 and an S/N of 10 is required. With the current assumptions, the atmospheric characterization of several Earth-like exoplanets at a distance of 10 pc and within a reasonable amount of observing time will require apertures $\geq2$ meters.

==> Konrad+(AstroPh)/Tables/Table_1.tex <==
\begin{table}
\caption{Jeffrey's scale \citep{Jeffreys:Theory_of_prob}.}% title of Table
\label{table:1}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{c c c}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
$\log_{10}\left(K\right)$ &Probability &Strength of Evidence\\    % table heading 
\hline 
   $<0$     &$<0.5$         &Support for $\mathcal{M}_2$\\
   $0-0.5$  &$0.5-0.75$     &Very weak support for $\mathcal{M}_1$\\
   $0.5-1$  &$0.75-0.91$    &Substantial support for $\mathcal{M}_1$\\
   $1-2$    &$0.91-0.99$    &Strong support for $\mathcal{M}_1$\\
   $>2$     &$>0.99$        &Decisive support for $\mathcal{M}_1$\\ 
\hline 
\end{tabular}
\tablefoot{Scale for the interpretation of the Bayes' factor $K=\mathcal{Z}_{\mathcal{M}_1}(\mathcal{D})/\mathcal{Z}_{\mathcal{M}_2}(\mathcal{D})$. The scale is symmetrical, which means that negative values correspond to very weak/substantial/strong/decisive support for $\mathcal{M}_2$.}
\end{table}

==> Konrad+(AstroPh)/Tables/Table_2.tex <==
\begin{table}[]


\caption{Line lists used throughout this study.}           % title of Table
\label{table:2}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lll}    % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Species & Database & References\\
\hline


\ce{CO2}    &ExoMol         &\citet{10.1093/mnras/staa1874}   \\
\ce{O3}     &HITRAN 2012    &\citet{2019AA...627A..67M};\\
            &               &\citet{2013JQSRT.130....4R} \\
\ce{CH4}    &ExoMol         &\citet{2021A...646A..21C};\\
            &               &\citet{10.1093/mnras/staa1874} \\
\ce{CO}     &HITEMP         &\citet{ROTHMAN20102139}   \\
\ce{H2O}    &HITEMP         &\citet{ROTHMAN20102139} \\
\ce{N2O}    &ExoMol         &\citet{2021A...646A..21C} \\
\hline 
\end{tabular}
\end{table}

==> Konrad+(AstroPh)/Tables/Table_3.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.5}

\caption{List of parameters used in the retrievals, their input values, prior distributions, and the validation results.}             % title of Table
\label{table:3}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{llllr}    % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Parameter &Description &Input &Prior & Validation \\    % table heading 
\hline

$\sqrt[4]{a_4}$ &P-T Parameter (Degree 4)  & $1.14$   & $\mathcal{U}(0.5,1.8)$ &$1.12^{+0.05}_{-0.04}$\\
$a_3$           &P-T parameter (Degree 3)  & $23.12$  & $\mathcal{U}(0,100)$  & $22.65^{+1.74}_{-1.54}$\\
$a_2$           &P-T Parameter (Degree 2)  & $99.70$  & $\mathcal{U}(0,500)$   & $98.90^{+3.72}_{-3.44}$\\
$a_1$           &P-T Parameter  (Degree 1) & $146.63$ & $\mathcal{U}(0,500)$   & $146.07^{+4.75}_{-4.84}$\\
$a_0$           &P-T Parameter (Degree 0) & $285.22$ & $\mathcal{U}(0,1000)$  & $285.01^{+3.16}_{-3.08}$\\


$\log_{10}\left(P_0\left[\mathrm{bar}\right]\right)$&Surface Pressure  & $0.006$\tablefootmark{1}  & $\mathcal{U}(-4,3)$& $0.01^{+0.02}_{-0.02}$\\
$R_{\text{pl}}\,\left[R_\oplus\right]$&Planet Radius& $1.0$  & $\mathcal{G}(1.0,0.2)$ & $1.00^{+0.01}_{-0.01}$\\ 
$\log_{10}\left(M_{\text{pl}}\,\left[M_\oplus\right]\right)$&Planet Mass & $0.0$  & $\mathcal{G}(0.0,0.4)$& $-0.09^{+0.18}_{-0.22}$\\

$\log_{10}(\mathrm{N_2})$    &\ce{N2}  Mass Fraction  & $-0.107$\tablefootmark{1,2} & $\mathcal{U}(-3,0)$  & $-0.14^{+0.09}_{-0.11}$\\
$\log_{10}(\mathrm{O_2})$    & \ce{O2} Mass Fraction     & $-0.679$\tablefootmark{1,2} & $\mathcal{U}(-3,0)$  & $-0.75^{+0.18}_{-0.17}$\\
$\log_{10}(\mathrm{H_2O})$   & \ce{H2O} Mass Fraction           & $-3.000$ & $\mathcal{U}(-15,0)$ & $-3.09^{+0.18}_{-0.22}$\\ 
$\log_{10}(\mathrm{CO_2})$   & \ce{CO2} Mass Fraction    & $-3.387$\tablefootmark{1,2} & $\mathcal{U}(-15,0)$ & $-3.47^{+0.18}_{-0.22}$\\
$\log_{10}(\mathrm{CH_4})$   & \ce{CH4} Mass Fraction          & $-5.770$\tablefootmark{1,2} & $\mathcal{U}(-15,0)$ & $-5.85^{+0.18}_{-0.23}$\\
$\log_{10}(\mathrm{O_3})$    & \ce{O3} Mass Fraction           & $-6.523$\tablefootmark{2} & $\mathcal{U}(-15,0)$ & $-6.61^{+0.18}_{-0.23}$\\
$\log_{10}(\mathrm{CO})$     &\ce{CO}  Mass Fraction      & $-6.903$\tablefootmark{2} & $\mathcal{U}(-15,0)$& $-7.02^{+0.23}_{-0.28}$\\
$\log_{10}(\mathrm{N_2O})$   &\ce{N2O} Mass Fraction    & $-6.495$\tablefootmark{2} & $\mathcal{U}(-15,0)$& $-6.60^{+0.24}_{-0.27}$\\
\hline 
\end{tabular}
\tablefoot{The last column shows the output value with 1$\sigma$ uncertainties for each parameter obtained in the validation run (Sect.~\ref{Validation}). $\mathcal{U}(x,y)$ denotes a boxcar prior with a lower threshold $x$ and upper threshold $y$; $\mathcal{G}(\mu,\sigma)$ represents a Gaussian prior with mean $\mu$ and standard deviation $\sigma$. For $a_4$ we choose a prior on $\sqrt[4]{a_4}$, which allows us to sample small values more densely, typical of a 4\textsuperscript{th} order coefficient, and then take the 4\textsuperscript{th} power to obtain $a_4$.}
\tablebib{\tablefoottext{1}{NASA's planet factsheet: \url{https://nssdc.gsfc.nasa.gov/planetary/factsheet/earthfact.html}}
\tablefoottext{2}{Table A1 in \citet{doi:10.1089/ast.2015.1404}}}
\end{table*}

==> Konrad+(AstroPh)/Tables/Table_4.tex <==
\bgroup
\def\arraystretch{1.3}%

\begin{table*}
\caption{Results obtained in the retrieval sensitivity analysis.}          
\label{table:4}      
\centering          
\begin{tabular}{lcccccccc}     % 7 columns 
\hline\hline       
                      % To combine 4 columns into a single one 
R & S/N &Range $\left[\mu\mathrm{m}\right]$ &$\mathrm{log_{10}\left(H_2O\right)}$ &$\mathrm{log_{10}\left(CO_2\right)}$ &$\mathrm{log_{10}\left(O_3\right)}$ &$\mathrm{log_{10}\left(CH_4\right)}$ &$\mathrm{log_{10}\left(CO\right)}$ &$\mathrm{log_{10}\left(N_2O\right)}$\\ 
\hline                    
\multirow{4}{*}{$20$} &\multirow{2}{*}{$10$}    &$3-20$ &$-6.13^{\pm0.38}$                              &$-6.51^{\pm0.33}$  &-7.22$^{\pm0.38}$   &$-6.04^{\pm0.51}$                         &$-4.14^{\pm1.32}$  &$-3.39^{\pm1.23}$   \\  
                    &                           &$6-17$ &$-6.11^{\pm0.54}$   &$-6.61^{\pm0.52}$  &$-7.04^{\pm0.30}$   &$-5.91^{\pm0.57}$ &UC                 &$-3.09^{\pm1.04}$   \\\cdashline{3-9}
                    &\multirow{2}{*}{$20$}      &$3-20$ &$-6.68^{\pm0.45}$   &$-7.08^{\pm0.48}$  &$-7.55^{\pm0.27}$   &$-6.68^{\pm0.53}$ &$-5.28^{\pm0.63}$  &$-4.55^{\pm1.05}$   \\
                    &                           &$6-17$ &$-6.63^{\pm0.40}$   &$-7.05^{\pm0.44}$  &$-7.47^{\pm0.37}$   &$-6.67^{\pm0.56}$ &UC                 &$-4.30^{\pm1.02}$   \\\cdashline{2-9}
\multirow{4}{*}{$50$} &\multirow{2}{*}{$10$}    &$3-20$ &$-6.60^{\pm0.49}$                              &$-7.08^{\pm0.52}$  &$-7.45^{\pm0.31}$   &$-6.49^{\pm0.42}$                         &$-5.26^{\pm0.67}$  &$-4.33^{\pm1.07}$   \\  
                    &                           &$6-17$ &$-6.47^{\pm0.45}$   &$-7.05^{\pm0.46}$  &$-7.46^{\pm0.28}$   &$-6.56^{\pm0.55}$   &UC                 &$-3.86^{\pm0.98}$   \\\cdashline{3-9}
                    &\multirow{2}{*}{$20$}      &$3-20$ &$-6.99^{\pm0.34}$   &$-7.48^{\pm0.34}$  &$-7.75^{\pm0.22}$   &$-7.09^{\pm0.45}$   &$-5.82^{\pm0.36}$  &$-5.28^{\pm0.75}$   \\
                    &                           &$6-17$ &$-6.98^{\pm0.34}$   &$-7.50^{\pm0.41}$  &$-7.84^{\pm0.36}$   &$-7.08^{\pm0.33}$   &UC                 &$-5.10^{\pm0.87}$   \\\cdashline{2-9}
$1000$&$50$&$3-20$&$-9.29^{\pm0.25}$&$-9.27^{\pm0.27}$&$-9.02^{\pm0.27}$&$-8.81^{\pm0.29}$&$-7.88^{\pm0.29}$&$-8.35^{\pm0.35}$\\
\hline 
\multicolumn{3}{l}{Terrestrial abundances:}&$-3.00$&$-3.39$&$-5.77$&$-6.52$&$-6.90$&$-6.50$\\
\multicolumn{3}{l}{\textit{LIFE} retrieval expectation:}&\textcolor{Green}{$\boldsymbol{\checkmark}$}&\textcolor{Green}{$\boldsymbol{\checkmark}$}&\textcolor{Green}{$\boldsymbol{\checkmark}$}&\textcolor{BurntOrange}{$\boldsymbol{\sim}$}&\textcolor{Red}{$\boldsymbol{\times}$}&\textcolor{Red}{$\boldsymbol{\times}$}\\\hline
\end{tabular}
\tablefoot{All abundances are given in mass fractions in $\log_{10}$. We provide the threshold abundances for a detection at different R and S/N configurations, which we define as the half maximum  of the retrieved soft step posterior distribution. Additionally, we provide the 16\textsuperscript{th} and 84\textsuperscript{th} percentile of the logistic function as denoted by the '$\pm$'. 'UC' stands for unconstrained and signifies that the retrieval does not manage to constrain the species of interest. In the last two rows, we display the assumed Earth-twin abundances and whether we expect such an abundance to be retrievable in low R and S/N cases, respectively: '\textcolor{Green}{$\boldsymbol{\checkmark}$}' $=$ retrievable; '\textcolor{BurntOrange}{$\boldsymbol{\sim}$}' $=$ case dependant; '\textcolor{Red}{$\boldsymbol{\times}$}' $=$ not retrievable.}
\end{table*}

\egroup

==> Konrad+(AstroPh)/Tables/Table_5.tex <==
\begin{table}
\caption{Log-evidence for retrievals with and without $\mathrm{CH_4}$.}


\begin{tabular}{ccc:ccc}
\hline\hline
\multicolumn{3}{c:}{S/N}                   & $10$              & $15$              & $20$  \\\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{$\begin{array}{c}\text{Nominal}\\\text{Case}\end{array}$}}&\multirow{3}{*}{\rotatebox[origin=c]{90}{${\mathrm{R}=35}$}} & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{CH_4})}$\end{tabular}                                                    & $-23.6^{\pm0.2}$  & $-27.0^{\pm0.2}$  & $-28.8^{\pm0.2}$                   \\
&& \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{-CH_4})}$\end{tabular}                                                                       & $-23.7^{\pm0.2}$                    & $-27.2^{\pm0.2}$                   & $-28.8^{\pm0.2}$                   \\
                        \cdashline{3-6}

&&\begin{tabular}[c]{@{}c@{}}$\mathrm{log_{10}\left(K\right)}$\end{tabular} & $0.0^{\pm0.1}$                      & $0.1^{\pm0.1}$                     & $0.0^{\pm0.1}$                      \\
                        \cline{2-6}
&\multirow{3}{*}{\rotatebox[origin=c]{90}{${\mathrm{R}=50}$}} & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{CH_4})}$\end{tabular}                                                                          & $-25.1^{\pm0.2}$                    & $-27.8^{\pm0.2}$                   & $-29.8^{\pm0.2}$              \\
&& \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{-CH_4})}$\end{tabular}                                                                     & $-25.4^{\pm0.2}$                    & $-28.4^{\pm0.2}$                   & $-30.6^{\pm0.2}$             \\\cdashline{3-6}
&                        &\begin{tabular}[c]{@{}c@{}}$\mathrm{log_{10}\left(K\right)}$\end{tabular} & $0.1^{\pm0.1}$                      & $0.3^{\pm0.1}$                     & $0.3^{\pm0.1}$          \\
                        \hline
                        
                        
                        
                        

\multirow{6}{*}{\rotatebox[origin=c]{90}{$\begin{array}{c}\mathrm{Optimized}\\\mathrm{Case}\end{array}$}}&\multirow{3}{*}{\rotatebox[origin=c]{90}{${\mathrm{R}=35}$}} & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{CH_4})}$\end{tabular}                                                                                             & $-24.8^{\pm0.2}$               & $-27.9^{\pm0.2}$               & $-30.2^{\pm0.2}$              \\
&                        & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{-CH_4})}$\end{tabular}                                                                                        & $-24.9^{\pm0.2}$               & $-28.2^{\pm0.2}$               & $-30.1^{\pm0.2}$              \\
                        \cdashline{3-6}

&&\begin{tabular}[c]{@{}c@{}}$\mathrm{log_{10}\left(K\right)}$\end{tabular}              & $0.0^{\pm0.1}$                 & $0.1^{\pm0.1}$                 & $0.0^{\pm0.1}$                \\
                        \cline{2-6}
&\multirow{3}{*}{\rotatebox[origin=c]{90}{${\mathrm{R}=50}$}} & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{CH_4})}$\end{tabular}                                                                              & $-26.7^{\pm0.2}$               & $-29.6^{\pm0.2}$               & $-31.5^{\pm0.2}$              \\
&                        & \begin{tabular}[c]{@{}c@{}}$\mathrm{ln(\mathcal{Z}_\mathrm{-CH_4})}$\end{tabular}                                                                              & $-28.8^{\pm0.2}$               & $-31.7^{\pm0.2}$               & $-35.1^{\pm0.2}$              \\\cdashline{3-6}
&                        &\begin{tabular}[c]{@{}c@{}}$\mathrm{log_{10}\left(K\right)}$\end{tabular}                    & $0.8^{\pm0.1}$                 & $0.9^{\pm0.1}$                 & $1.6^{\pm0.1}$      \\
                        \hline
                         
\end{tabular}

\label{table:5}
\tablefoot{With $\mathrm{CH_4}$: $\mathrm{ln}(\mathcal{Z}_\mathrm{CH_4})$; Without $\mathrm{CH_4}$: $\mathrm{ln}(\mathcal{Z}_\mathrm{-CH_4})$. The results are for input spectra covering the $3-20\,\mu\mathrm{m}$ wavelength range. The last row for a given R lists $\mathrm{log}_{10}\left(K\right)$ of the Bayes' factor $K$, which we calculate via: $\mathrm{log}_{10}\left(K\right)=\left(\ln\left(\mathcal{Z}_\mathrm{CH_4}\right)-\ln\left({\mathcal{Z}_\mathrm{-CH_4}}\right)\right) /\ln\left(10\right)$ (derived from Eq. \ref{equ:bayes_factor}). We compare the performance of the models with and without $\mathrm{CH_4}$ to each other using Jeffrey's scale \citep{Jeffreys:Theory_of_prob} (see Table \ref{table:1}). The '${\pm}$' indicates the $68\%$ confidence interval $\mathrm{log}_{10}\left(K\right)$.}
\end{table}









==> Konrad+(AstroPh)/Tables/Table_6.tex <==
\begin{table}
\caption{Required observation time in days.}            % title of Table
\label{table:6}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{c c:c c c: c c c}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{6}{c}{Observation Time [days]}\\
& &\multicolumn{3}{c:}{Nominal Case} &\multicolumn{3}{c}{Optimized Case}\\
R&S/N &1 m&2 m&3.5 m&1 m&2 m&3.5 m\\% table heading 
\hline 
$35$    &$15$  &$771$   &$74$   &$15$   &$922$  &$64$   &$9$  \\

$50$    &$10$  &$490$   &$47$   &$10$   &$589$  &$41$   &$6$  \\
\hline 
\end{tabular}
\tablefoot{Observation times for an Earth-twin at 10 pc for the two combinations of R and S/N discussed in Sect.~\ref{sec:Baselines} and three different aperture diameters (1m, 2m, and 3.5m). We conservatively assume a total instrument throughput of 5\% \citep[cf.][]{dannert2022large}.}
\end{table}

==> Konrad+(AstroPh)/Tables/Table_Integration_Times.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Integration times optimized for short wavelengths

\begin{table}[h]
\centering

\caption{Required observation time in days.}

\subfloat[Nominal case]{
\begin{tabular}{clc:cccc}
\hline\hline
&&&\multicolumn{4}{c}{Observation Time [days]}\\
\multicolumn{3}{c:}{R}   & 20       & 35        & 50        & 100       \\ \hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{S/N}} & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}1 m\\Mirrors\end{tabular}}}   &5  & 48.6   & 85.7    & 122.5   & 249.1   \\ 
                                        &                                     &10 & 194.6  & 342.7   & 490.1   & 996.2  \\
                                        &                                     &15 & 437.8  & 771.0   & 1102.7  & 2241.5  \\ 
                                        &                                     &20 & 778.3  & 1370.6  & 1960.4  & 3984.8  \\ \cline{2-7} 
                                        & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}2 m\\Mirrors\end{tabular}}}   & 5                       & 4.7    & 8.2    & 11.7    & 23.9    \\
                                        &                                     & 10                      & 18.6   & 32.7    & 46.7    & 95.4   \\
                                        &                                     & 15                      & 41.9   & 73.5    & 105.0   & 214.7   \\
                                        &                                     & 20                      & 74.5   & 130.7  & 186.6   & 381.7   \\ \cline{2-7} 
                                        & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}3.5 m\\Mirrors\end{tabular}}} & 5                       & 1.0    & 1.7     & 2.4     & 4.9     \\
                                        &                                     & 10                      & 3.8    & 6.7    & 9.5    & 19.6    \\
                                        &                                     & 15                      & 8.6    & 15.1    & 21.5    & 44.2    \\
                                        &                                     & 20                      & 15.3   & 26.8    & 38.2    & 78.5    \\ \hline
\end{tabular}}

\subfloat[Optimized case]{
\begin{tabular}{clc:cccc}
\hline\hline
&&&\multicolumn{4}{c}{Observation Time [days]}\\
\multicolumn{3}{c:}{R}   & 20       & 35        & 50        & 100       \\ \hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{S/N}} & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}1m\\Mirrors\end{tabular}}}   &5  & 57.7   & 102.5    & 147.1   & 294.7   \\ 
                                        &                                     &10 & 230.6  & 410.0   & 588.5   & 1178.7  \\
                                        &                                     &15 & 518.9  & 922.2   & 1324.2  & 2652.2  \\ 
                                        &                                     &20 & 922.5  & 1639.5  & 2354.1  & 4714.9  \\ \cline{2-7}
                                        & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}2m\\Mirrors\end{tabular}}}   & 5                       & 4.0    & 7.1     & 10.2    & 20.6    \\
                                        &                                     & 10                      & 16.0   & 28.5    & 41.0    & 82.3   \\ 
                                        &                                     & 15                      & 36.2   & 64.2   & 92.1   & 185.2   \\
                                        &                                     & 20                      & 64.4   & 114.2  & 163.8   & 329.2  \\\cline{2-7} 
                                        & \multirow{4}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{cc}3.5m\\Mirrors\end{tabular}}} & 5                       & 0.6    & 1.0     & 1.4     & 2.9     \\ 
                                        &                                     & 10                      & 2.2    & 3.9    & 5.7   & 11.4   \\
                                        &                                     & 15                      & 5.0   & 8.9    & 12.7    & 25.7   \\
                                        &                                     & 20                      & 8.9   & 15.8    & 22.6    & 45.8    \\ \hline
\end{tabular}}
\tablefoot{Observation times necessary for \textit{LIFE} to investigate an Earth-twin at 10 pc in orbit around a G$2$ star for the grid of R and S/N discussed in this publication. The S/N in the Table corresponds to the S/N at $11.2\,\mu\mathrm{m}$. We consider three different aperture diameters (1m, 2m, and 3.5m) and conservatively assume a total instrument throughput of 5\% \citep[cf.][]{dannert2022large}.  (a): Nominal case; (b): Optimized case.}
\label{tab:all_integration_times}
\end{table}

==> Konrad+(AstroPh)/Tables/Table_PT_Priors.tex <==
\begin{table}
\caption{Priors used in the P-T profile retrievals.}
\label{tab:Priors_PT_Retrieval}
\centering
\begin{tabular}{ccc}
\hline\hline
Model                  &Model Parameter                  &Prior                \\ \hline
Polynomial                      & $a_i$                                     & $\mathcal{U}(-1000,1000)$     \\ \hdashline
Madhusudhan                     & $\mathrm{log}_{10}\left(P_i\right)$                & $\mathcal{U}(-10,4)$          \\
\& Seager                       & $T_0$                                     & $\mathcal{U}(0,1000)$         \\
                                & $\alpha_1, \alpha_2$                      & $\mathcal{U}(0,100)$          \\ \hdashline
Guillot                   & $T_{equ}$, $T_{int}$                      & $\mathcal{U}(0,1000)$         \\
                                & $\kappa_{IR}$                             & $\mathcal{U}(0,1)$            \\
                                & $\gamma$                                  & $\mathcal{U}(0,100)$          \\
                                \hdashline 
Addition for                    & $\mathrm{log}_{10}\left(P_{Trans}\right)$          & $\mathcal{U}(-10,4)$          \\
Modified Guillot                & $\alpha$                                  & $\mathcal{U}(-1,1)$           \\ \hline

\end{tabular}
\tablefoot{$\mathcal{U}(x,y)$: boxcar prior with lower limit $x$ and upper limit $y$.}
\end{table}

==> Konrad+(AstroPh)/Tables/Table_Ret_Results.tex <==
\bgroup
\def\arraystretch{1.5}%
\begin{table*}[]
\caption{Retrieval results for the $3-20\,\mu$m wavelength range for the nominal case.}           % title of Table
\label{table:3-20}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.2_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.3_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$34.3_{-19.4}^{+29.5}$&$15.8_{-8.0}^{+13.0}$&$13.2_{-6.6}^{+9.3}$&$13.3_{-6.7}^{+11.2}$&$26.7_{-14.2}^{+21.3}$&$14.7_{-7.2}^{+11.2}$&$14.2_{-7.0}^{+11.6}$&$13.7_{-6.2}^{+10.1}$\\ 

$a_2$&99.70&$163.8_{-80.0}^{+114.4}$&$65.0_{-33.3}^{+49.7}$&$56.0_{-30.0}^{+38.9}$&$52.4_{-25.7}^{+37.2}$&$102.3_{-48.4}^{+63.0}$&$57.2_{-27.4}^{+35.5}$&$57.4_{-24.9}^{+33.5}$&$57.8_{-21.7}^{+29.9}$\\ 

$a_1$&146.63&$147.5_{-76.7}^{+125.6}$&$104.1_{-44.5}^{+71.1}$&$99.2_{-38.5}^{+68.4}$&$80.3_{-31.3}^{+62.4}$&$108.0_{-50.5}^{+68.6}$&$90.3_{-28.8}^{+47.1}$&$87.6_{-31.1}^{+46.5}$&$88.3_{-32.5}^{+56.0}$\\ 

$a_0$&285.22&$234.2_{-93.5}^{+94.6}$&$281.4_{-42.3}^{+45.3}$&$288.1_{-34.3}^{+45.7}$&$266.5_{-26.2}^{+34.6}$&$240.1_{-54.8}^{+42.8}$&$276.3_{-29.7}^{+34.1}$&$269.8_{-27.2}^{+33.0}$&$266.6_{-26.1}^{+43.3}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.4_{-0.5}^{+0.3}$&$0.1_{-0.4}^{+0.4}$&$-0.0_{-0.4}^{+0.4}$&$0.2_{-0.3}^{+0.3}$&$0.4_{-0.3}^{+0.2}$&$0.1_{-0.3}^{+0.3}$&$0.2_{-0.3}^{+0.3}$&$0.2_{-0.4}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.82_{-0.1}^{+0.1}$&$0.96_{-0.09}^{+0.09}$&$1.01_{-0.08}^{+0.08}$&$1.02_{-0.07}^{+0.06}$&$0.88_{-0.10}^{+0.10}$&$0.99_{-0.08}^{+0.08}$&$1.01_{-0.06}^{+0.06}$&$1.03_{-0.05}^{+0.05}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.1_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.3_{-4.4}^{+4.1}$&$-7.8_{-4.2}^{+4.6}$&$-7.6_{-4.5}^{+4.6}$&$-7.6_{-4.5}^{+4.5}$&$-7.5_{-4.3}^{+4.4}$&$-7.4_{-4.4}^{+4.4}$&$-7.7_{-4.4}^{+4.6}$&$-7.8_{-4.4}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.0_{-4.6}^{+4.2}$&$-7.1_{-4.6}^{+4.4}$&$-7.4_{-4.5}^{+4.5}$&$-7.5_{-4.7}^{+4.6}$&$-7.7_{-4.3}^{+4.5}$&$-7.4_{-4.6}^{+4.3}$&$-7.6_{-4.5}^{+4.5}$&$-7.5_{-4.8}^{+4.7}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-9.4_{-3.4}^{+3.8}$&$-3.2_{-1.1}^{+1.1}$&$-2.7_{-0.8}^{+0.9}$&$-3.1_{-0.7}^{+0.7}$&$-5.3_{-5.2}^{+1.7}$&$-2.9_{-0.8}^{+0.8}$&$-3.0_{-0.7}^{+0.7}$&$-3.0_{-0.7}^{+0.8}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-6.6_{-4.8}^{+1.9}$&$-3.6_{-0.8}^{+0.9}$&$-3.2_{-0.7}^{+0.7}$&$-3.6_{-0.6}^{+0.7}$&$-4.6_{-1.0}^{+0.8}$&$-3.4_{-0.7}^{+0.8}$&$-3.5_{-0.6}^{+0.7}$&$-3.5_{-0.6}^{+0.7}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.9_{-3.0}^{+3.1}$&$-8.7_{-3.8}^{+3.2}$&$-9.2_{-3.6}^{+3.4}$&$-9.6_{-3.2}^{+3.3}$&$-9.2_{-3.3}^{+3.4}$&$-9.7_{-3.2}^{+3.6}$&$-9.3_{-3.3}^{+3.2}$&$-9.0_{-3.8}^{+2.8}$\\ 

$L(\mathrm{O_3})$&-6.523&$-10.3_{-2.8}^{+2.7}$&$-6.8_{-2.2}^{+0.9}$&$-6.4_{-0.6}^{+0.6}$&$-6.7_{-0.5}^{+0.5}$&$-9.6_{-3.3}^{+2.5}$&$-6.5_{-0.6}^{+0.6}$&$-6.6_{-0.5}^{+0.5}$&$-6.7_{-0.5}^{+0.6}$\\ 

$L(\mathrm{CO})$&-6.903&$-9.8_{-3.0}^{+3.3}$&$-7.8_{-4.3}^{+4.3}$&$-7.5_{-4.5}^{+4.3}$&$-7.7_{-4.3}^{+4.5}$&$-8.7_{-3.7}^{+4.0}$&$-7.7_{-4.2}^{+4.3}$&$-7.7_{-4.4}^{+4.4}$&$-7.7_{-4.5}^{+4.3}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-10.3_{-2.6}^{+2.8}$&$-8.5_{-3.9}^{+3.8}$&$-8.1_{-3.9}^{+3.7}$&$-8.5_{-4.0}^{+3.6}$&$-9.4_{-3.2}^{+3.5}$&$-8.3_{-3.9}^{+3.6}$&$-8.7_{-3.9}^{+3.6}$&$-8.9_{-3.7}^{+3.4}$\\ 
\hline
\multicolumn{10}{c}{} \\


\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.2_{-0.2}^{+0.3}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.3}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$22.2_{-10.6}^{+29.6}$&$14.4_{-7.4}^{+11.8}$&$18.0_{-8.4}^{+20.9}$&$15.3_{-6.3}^{+11.2}$&$12.9_{-6.6}^{+10.0}$&$14.1_{-6.2}^{+11.4}$&$16.2_{-6.6}^{+12.1}$&$19.3_{-8.4}^{+16.8}$\\ 

$a_2$&99.70&$94.0_{-41.9}^{+69.0}$&$61.6_{-29.0}^{+43.5}$&$76.6_{-33.1}^{+69.7}$&$71.8_{-26.9}^{+34.7}$&$47.8_{-21.8}^{+26.9}$&$62.6_{-24.5}^{+35.2}$&$73.5_{-22.7}^{+34.7}$&$88.6_{-30.0}^{+56.3}$\\ 

$a_1$&146.63&$120.6_{-47.8}^{+72.6}$&$102.0_{-38.2}^{+70.2}$&$134.5_{-69.7}^{+83.4}$&$114.0_{-42.8}^{+81.2}$&$70.3_{-24.8}^{+33.5}$&$101.3_{-42.1}^{+64.2}$&$115.4_{-36.3}^{+68.2}$&$154.1_{-62.4}^{+68.0}$\\ 

$a_0$&285.22&$265.1_{-41.7}^{+47.0}$&$285.1_{-34.3}^{+39.9}$&$294.1_{-44.8}^{+49.0}$&$280.4_{-32.2}^{+61.1}$&$256.0_{-24.4}^{+30.6}$&$273.9_{-30.8}^{+45.1}$&$279.2_{-26.3}^{+47.7}$&$298.8_{-38.8}^{+41.7}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.2_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.4}$&$-0.1_{-0.3}^{+0.5}$&$0.0_{-0.4}^{+0.3}$&$0.3_{-0.3}^{+0.3}$&$0.1_{-0.4}^{+0.4}$&$0.0_{-0.3}^{+0.3}$&$-0.1_{-0.2}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.92_{-0.09}^{+0.09}$&$1.01_{-0.07}^{+0.07}$&$1.03_{-0.05}^{+0.06}$&$1.03_{-0.05}^{+0.05}$&$0.98_{-0.08}^{+0.08}$&$1.02_{-0.06}^{+0.06}$&$1.02_{-0.04}^{+0.04}$&$1.01_{-0.03}^{+0.04}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-6.5_{-4.6}^{+4.0}$&$-7.6_{-4.5}^{+4.5}$&$-7.3_{-4.7}^{+4.4}$&$-7.6_{-4.5}^{+4.7}$&$-7.9_{-4.1}^{+4.5}$&$-7.9_{-4.5}^{+4.8}$&$-7.4_{-4.6}^{+4.4}$&$-7.4_{-4.7}^{+4.6}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.8_{-4.3}^{+4.5}$&$-7.2_{-4.5}^{+4.4}$&$-7.1_{-4.7}^{+4.5}$&$-7.5_{-4.5}^{+4.7}$&$-7.4_{-4.4}^{+4.2}$&$-7.8_{-4.3}^{+5.0}$&$-7.3_{-4.7}^{+4.5}$&$-7.5_{-4.6}^{+4.6}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-3.7_{-2.1}^{+1.1}$&$-2.8_{-0.8}^{+0.8}$&$-2.7_{-0.8}^{+0.7}$&$-2.8_{-0.7}^{+0.8}$&$-3.6_{-0.8}^{+0.9}$&$-3.0_{-0.8}^{+0.8}$&$-2.9_{-0.6}^{+0.6}$&$-2.7_{-0.6}^{+0.5}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-4.0_{-0.8}^{+0.8}$&$-3.3_{-0.7}^{+0.7}$&$-3.2_{-0.7}^{+0.7}$&$-3.3_{-0.7}^{+0.7}$&$-3.9_{-0.7}^{+0.8}$&$-3.4_{-0.7}^{+0.7}$&$-3.3_{-0.5}^{+0.6}$&$-3.2_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-8.5_{-3.8}^{+3.1}$&$-9.0_{-3.6}^{+3.1}$&$-8.8_{-3.7}^{+2.9}$&$-7.7_{-4.4}^{+2.1}$&$-9.5_{-3.3}^{+3.2}$&$-8.7_{-3.7}^{+2.7}$&$-6.8_{-4.2}^{+1.3}$&$-5.9_{-1.4}^{+0.7}$\\ 

$L(\mathrm{O_3})$&-6.523&$-7.7_{-4.1}^{+1.4}$&$-6.5_{-0.6}^{+0.6}$&$-6.5_{-0.6}^{+0.6}$&$-6.5_{-0.5}^{+0.5}$&$-7.0_{-0.7}^{+0.7}$&$-6.6_{-0.5}^{+0.6}$&$-6.5_{-0.4}^{+0.4}$&$-6.4_{-0.4}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.8_{-4.0}^{+4.0}$&$-7.8_{-4.3}^{+4.5}$&$-7.7_{-4.5}^{+4.4}$&$-7.9_{-4.3}^{+4.4}$&$-8.1_{-4.0}^{+4.5}$&$-7.7_{-4.5}^{+4.7}$&$-7.8_{-4.4}^{+4.6}$&$-8.0_{-4.4}^{+4.6}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.0_{-3.4}^{+3.8}$&$-8.5_{-3.8}^{+3.7}$&$-8.7_{-3.9}^{+3.5}$&$-8.9_{-3.7}^{+3.4}$&$-9.1_{-3.4}^{+3.5}$&$-9.0_{-3.7}^{+3.6}$&$-9.0_{-3.6}^{+3.4}$&$-9.3_{-3.7}^{+3.5}$\\ 
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}












\begin{table*}
\caption{Retrieval results for the $3-20\,\mu$m wavelength range for the optimized case.}            % title of Table
\label{table:3-20_opt}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline

$\sqrt[4]{a_4}$&1.14&$1.2_{-0.3}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$25.5_{-12.3}^{+20.0}$&$14.2_{-6.7}^{+9.4}$&$10.7_{-5.3}^{+8.0}$&$13.2_{-6.4}^{+11.7}$&$16.4_{-8.2}^{+14.3}$&$10.6_{-5.1}^{+7.1}$&$11.5_{-5.4}^{+10.3}$&$11.8_{-5.0}^{+8.2}$\\ 

$a_2$&99.70&$108.3_{-41.4}^{+59.0}$&$60.4_{-27.5}^{+36.3}$&$38.9_{-20.8}^{+30.2}$&$61.3_{-32.6}^{+51.6}$&$64.1_{-30.6}^{+41.2}$&$43.3_{-22.8}^{+33.8}$&$47.0_{-21.8}^{+36.5}$&$50.0_{-20.2}^{+26.1}$\\ 

$a_1$&146.63&$128.8_{-60.6}^{+67.5}$&$105.4_{-37.0}^{+51.8}$&$71.4_{-25.9}^{+42.2}$&$130.8_{-60.7}^{+97.0}$&$86.5_{-43.8}^{+56.6}$&$91.4_{-31.0}^{+53.7}$&$89.4_{-32.5}^{+59.0}$&$89.1_{-30.6}^{+42.1}$\\ 

$a_0$&285.22&$201.5_{-73.0}^{+73.6}$&$266.4_{-33.2}^{+42.4}$&$266.6_{-27.8}^{+33.0}$&$323.4_{-45.3}^{+66.8}$&$227.9_{-59.1}^{+46.2}$&$294.7_{-37.9}^{+40.7}$&$285.8_{-32.5}^{+43.6}$&$277.9_{-24.8}^{+29.5}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.5_{-0.4}^{+0.3}$&$0.2_{-0.4}^{+0.3}$&$0.2_{-0.4}^{+0.4}$&$-0.3_{-0.3}^{+0.4}$&$0.6_{-0.4}^{+0.3}$&$-0.1_{-0.4}^{+0.4}$&$0.0_{-0.4}^{+0.4}$&$0.1_{-0.3}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.9_{-0.1}^{+0.1}$&$0.99_{-0.09}^{+0.09}$&$1.01_{-0.06}^{+0.07}$&$1.02_{-0.05}^{+0.06}$&$0.9_{-0.1}^{+0.1}$&$1.01_{-0.07}^{+0.07}$&$1.02_{-0.05}^{+0.05}$&$1.02_{-0.04}^{+0.04}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.6_{-4.2}^{+4.3}$&$-7.9_{-4.2}^{+4.5}$&$-7.7_{-4.5}^{+4.4}$&$-7.8_{-4.3}^{+4.7}$&$-7.6_{-4.3}^{+4.2}$&$-7.2_{-4.6}^{+4.2}$&$-7.5_{-4.5}^{+4.6}$&$-7.5_{-4.4}^{+4.6}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.0_{-4.6}^{+4.8}$&$-7.3_{-4.6}^{+4.4}$&$-7.1_{-4.3}^{+4.3}$&$-7.9_{-4.3}^{+4.5}$&$-7.1_{-4.5}^{+4.2}$&$-7.8_{-4.4}^{+4.6}$&$-7.4_{-4.5}^{+4.4}$&$-7.5_{-4.5}^{+4.6}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-4.2_{-3.0}^{+1.1}$&$-2.9_{-0.8}^{+0.9}$&$-2.9_{-0.8}^{+0.8}$&$-1.7_{-0.9}^{+0.7}$&$-3.8_{-0.9}^{+1.0}$&$-2.1_{-1.0}^{+0.9}$&$-2.4_{-0.9}^{+0.9}$&$-2.7_{-0.6}^{+0.7}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-6.6_{-4.6}^{+2.0}$&$-3.9_{-0.9}^{+0.9}$&$-3.7_{-0.8}^{+0.8}$&$-2.6_{-0.8}^{+0.6}$&$-5.1_{-2.4}^{+1.2}$&$-3.1_{-0.9}^{+0.9}$&$-3.1_{-0.8}^{+0.8}$&$-3.3_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.8_{-3.0}^{+2.8}$&$-9.9_{-3.1}^{+3.1}$&$-9.5_{-3.4}^{+3.0}$&$-7.9_{-4.1}^{+2.6}$&$-10.2_{-2.8}^{+2.8}$&$-9.4_{-3.3}^{+3.1}$&$-8.0_{-4.2}^{+2.2}$&$-6.5_{-4.0}^{+0.9}$\\ 

$L(\mathrm{O_3})$&-6.523&$-9.7_{-3.0}^{+2.3}$&$-6.7_{-0.7}^{+0.7}$&$-6.6_{-0.6}^{+0.6}$&$-5.9_{-0.6}^{+0.6}$&$-7.5_{-2.7}^{+0.8}$&$-6.2_{-0.7}^{+0.7}$&$-6.3_{-0.6}^{+0.6}$&$-6.5_{-0.4}^{+0.5}$\\ 

$L(\mathrm{CO})$&-6.903&$-9.0_{-3.6}^{+3.9}$&$-7.5_{-4.5}^{+4.4}$&$-7.8_{-4.5}^{+4.5}$&$-7.9_{-4.3}^{+4.5}$&$-8.3_{-3.9}^{+3.9}$&$-7.5_{-4.5}^{+4.4}$&$-7.7_{-4.4}^{+4.4}$&$-8.1_{-4.4}^{+4.3}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.8_{-3.0}^{+3.3}$&$-8.9_{-3.6}^{+3.7}$&$-9.0_{-3.6}^{+3.6}$&$-8.3_{-3.9}^{+3.4}$&$-8.8_{-3.5}^{+3.4}$&$-8.8_{-3.7}^{+3.8}$&$-9.4_{-3.3}^{+3.8}$&$-9.4_{-3.4}^{+3.3}$\\ 

\hline
\multicolumn{10}{c}{} \\

\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.3_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$30.4_{-13.0}^{+16.3}$&$14.1_{-6.7}^{+11.0}$&$11.7_{-5.1}^{+9.5}$&$13.9_{-6.2}^{+9.7}$&$10.7_{-5.1}^{+7.6}$&$14.7_{-6.4}^{+10.1}$&$19.1_{-8.4}^{+18.2}$&$17.0_{-6.7}^{+10.6}$\\ 

$a_2$&99.70&$112.7_{-41.3}^{+47.3}$&$64.4_{-30.6}^{+41.8}$&$43.8_{-18.1}^{+25.2}$&$53.2_{-19.9}^{+28.0}$&$40.3_{-21.0}^{+31.5}$&$67.9_{-26.6}^{+38.4}$&$86.6_{-37.8}^{+59.2}$&$78.0_{-26.9}^{+41.7}$\\ 

$a_1$&146.63&$141.1_{-54.4}^{+81.8}$&$126.8_{-44.3}^{+72.6}$&$69.1_{-20.7}^{+32.7}$&$79.3_{-27.2}^{+37.2}$&$79.7_{-33.1}^{+55.1}$&$128.1_{-46.1}^{+72.9}$&$148.4_{-72.5}^{+81.3}$&$132.2_{-56.2}^{+61.8}$\\ 

$a_0$&285.22&$255.5_{-41.8}^{+48.8}$&$311.1_{-31.6}^{+52.0}$&$260.9_{-19.7}^{+23.3}$&$260.8_{-19.2}^{+22.6}$&$273.8_{-32.1}^{+44.5}$&$306.9_{-39.7}^{+56.2}$&$298.4_{-42.5}^{+54.4}$&$286.7_{-34.3}^{+39.6}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.2_{-0.3}^{+0.2}$&$-0.2_{-0.3}^{+0.3}$&$0.3_{-0.3}^{+0.2}$&$0.3_{-0.2}^{+0.3}$&$0.1_{-0.4}^{+0.4}$&$-0.2_{-0.3}^{+0.4}$&$-0.1_{-0.3}^{+0.4}$&$-0.0_{-0.2}^{+0.4}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.98_{-0.09}^{+0.09}$&$1.02_{-0.06}^{+0.06}$&$1.01_{-0.04}^{+0.05}$&$1.01_{-0.03}^{+0.03}$&$1.01_{-0.08}^{+0.08}$&$1.01_{-0.04}^{+0.05}$&$1.0_{-0.03}^{+0.03}$&$1.0_{-0.02}^{+0.02}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.1_{-0.3}^{+0.2}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.8_{-4.0}^{+4.2}$&$-7.7_{-4.3}^{+4.7}$&$-7.8_{-4.4}^{+4.6}$&$-7.1_{-4.5}^{+4.2}$&$-7.3_{-4.8}^{+4.5}$&$-7.4_{-4.6}^{+4.6}$&$-7.5_{-4.7}^{+4.6}$&$-7.1_{-4.9}^{+4.5}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.1_{-4.2}^{+4.2}$&$-7.6_{-4.6}^{+4.5}$&$-7.5_{-4.6}^{+4.5}$&$-7.4_{-4.7}^{+4.6}$&$-7.2_{-4.6}^{+4.3}$&$-7.1_{-4.7}^{+4.4}$&$-7.7_{-4.5}^{+4.8}$&$-7.9_{-4.2}^{+5.0}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-3.2_{-0.7}^{+0.8}$&$-2.0_{-0.7}^{+0.7}$&$-3.2_{-0.6}^{+0.7}$&$-3.3_{-0.6}^{+0.6}$&$-2.8_{-0.9}^{+1.1}$&$-2.4_{-0.8}^{+0.8}$&$-2.8_{-0.7}^{+0.6}$&$-2.9_{-0.6}^{+0.5}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-4.2_{-1.0}^{+0.8}$&$-2.9_{-0.7}^{+0.7}$&$-3.7_{-0.5}^{+0.6}$&$-3.7_{-0.5}^{+0.5}$&$-3.5_{-0.9}^{+1.0}$&$-2.9_{-0.7}^{+0.7}$&$-3.2_{-0.6}^{+0.6}$&$-3.3_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.5_{-3.0}^{+2.9}$&$-8.0_{-4.4}^{+2.6}$&$-6.6_{-3.3}^{+0.7}$&$-6.2_{-0.6}^{+0.5}$&$-8.9_{-3.8}^{+2.8}$&$-5.7_{-1.1}^{+0.9}$&$-5.7_{-0.7}^{+0.6}$&$-5.8_{-0.6}^{+0.5}$\\ 

$L(\mathrm{O_3})$&-6.523&$-7.0_{-0.9}^{+0.6}$&$-6.1_{-0.5}^{+0.5}$&$-6.7_{-0.4}^{+0.4}$&$-6.7_{-0.4}^{+0.4}$&$-6.6_{-0.6}^{+0.8}$&$-6.2_{-0.5}^{+0.6}$&$-6.4_{-0.5}^{+0.5}$&$-6.5_{-0.4}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.8_{-4.1}^{+4.3}$&$-8.0_{-4.4}^{+4.6}$&$-8.0_{-4.2}^{+4.5}$&$-8.2_{-4.0}^{+4.5}$&$-7.9_{-4.6}^{+4.6}$&$-7.8_{-4.4}^{+4.3}$&$-8.6_{-4.0}^{+4.4}$&$-8.5_{-4.1}^{+4.1}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.8_{-3.0}^{+3.6}$&$-8.3_{-3.9}^{+3.5}$&$-9.3_{-3.4}^{+3.2}$&$-9.5_{-3.5}^{+3.2}$&$-8.5_{-3.9}^{+3.7}$&$-9.0_{-3.6}^{+3.6}$&$-9.4_{-3.5}^{+3.2}$&$-9.7_{-3.2}^{+3.2}$\\ 
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}


















\begin{table*}
\caption{Retrieval results for the $4-18.5\,\mu$m wavelength range for the nominal case.}       % title of Table
\label{table:4-18.5}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.3_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$39.3_{-22.0}^{+28.4}$&$15.1_{-7.1}^{+10.1}$&$14.9_{-7.4}^{+13.0}$&$11.7_{-5.7}^{+10.5}$&$18.9_{-9.3}^{+17.0}$&$12.1_{-5.9}^{+10.1}$&$12.6_{-5.8}^{+9.7}$&$13.5_{-6.5}^{+11.1}$\\ 

$a_2$&99.70&$192.8_{-90.8}^{+137.4}$&$60.8_{-28.7}^{+34.4}$&$59.1_{-29.8}^{+46.5}$&$45.3_{-22.1}^{+37.7}$&$85.3_{-41.0}^{+58.3}$&$53.4_{-26.3}^{+36.6}$&$52.4_{-24.2}^{+28.2}$&$57.6_{-24.2}^{+35.7}$\\ 

$a_1$&146.63&$176.0_{-90.0}^{+176.3}$&$98.3_{-31.5}^{+38.2}$&$99.4_{-35.8}^{+60.6}$&$80.5_{-31.1}^{+56.6}$&$127.6_{-60.3}^{+89.4}$&$103.3_{-36.5}^{+53.6}$&$84.0_{-32.6}^{+47.5}$&$93.0_{-33.2}^{+55.1}$\\ 

$a_0$&285.22&$272.1_{-107.3}^{+93.4}$&$267.3_{-30.9}^{+32.8}$&$280.4_{-31.4}^{+40.9}$&$275.1_{-33.0}^{+41.1}$&$265.1_{-53.7}^{+59.5}$&$291.7_{-33.7}^{+44.0}$&$270.0_{-28.4}^{+33.3}$&$273.6_{-26.8}^{+36.6}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.1_{-0.5}^{+0.5}$&$0.2_{-0.3}^{+0.2}$&$0.0_{-0.3}^{+0.3}$&$0.1_{-0.4}^{+0.4}$&$0.2_{-0.4}^{+0.4}$&$-0.1_{-0.4}^{+0.4}$&$0.2_{-0.3}^{+0.4}$&$0.1_{-0.3}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.86_{-0.09}^{+0.1}$&$0.99_{-0.1}^{+0.1}$&$1.01_{-0.08}^{+0.07}$&$1.03_{-0.06}^{+0.06}$&$0.9_{-0.1}^{+0.1}$&$1.01_{-0.08}^{+0.08}$&$1.02_{-0.06}^{+0.06}$&$1.03_{-0.05}^{+0.05}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.1_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.6_{-4.2}^{+4.2}$&$-7.4_{-4.4}^{+4.4}$&$-7.6_{-4.5}^{+4.7}$&$-7.1_{-4.7}^{+4.2}$&$-7.0_{-4.3}^{+4.0}$&$-7.2_{-4.7}^{+4.5}$&$-7.2_{-4.9}^{+4.5}$&$-7.4_{-4.7}^{+4.6}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.4_{-4.5}^{+4.5}$&$-7.6_{-4.5}^{+4.5}$&$-7.7_{-4.3}^{+4.5}$&$-7.2_{-4.5}^{+4.5}$&$-8.0_{-4.2}^{+4.6}$&$-8.0_{-4.4}^{+4.4}$&$-8.0_{-4.4}^{+4.8}$&$-7.5_{-4.8}^{+4.5}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-9.5_{-3.2}^{+4.1}$&$-3.2_{-0.8}^{+0.9}$&$-2.7_{-0.8}^{+0.8}$&$-2.7_{-0.9}^{+0.9}$&$-3.8_{-1.6}^{+1.4}$&$-2.5_{-0.9}^{+0.9}$&$-2.9_{-0.8}^{+0.8}$&$-2.8_{-0.7}^{+0.7}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-9.2_{-3.5}^{+3.7}$&$-3.8_{-0.8}^{+0.8}$&$-3.4_{-0.7}^{+0.8}$&$-3.4_{-0.7}^{+0.8}$&$-4.3_{-1.3}^{+1.1}$&$-3.2_{-0.8}^{+0.9}$&$-3.5_{-0.7}^{+0.7}$&$-3.4_{-0.6}^{+0.7}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-10.2_{-2.8}^{+2.9}$&$-9.5_{-3.4}^{+3.3}$&$-9.2_{-3.5}^{+3.1}$&$-9.2_{-3.5}^{+3.1}$&$-9.2_{-3.3}^{+3.1}$&$-9.5_{-3.4}^{+3.4}$&$-9.0_{-3.5}^{+2.9}$&$-8.0_{-4.3}^{+2.1}$\\ 

$L(\mathrm{O_3})$&-6.523&$-10.5_{-2.5}^{+2.6}$&$-7.0_{-3.5}^{+0.8}$&$-6.4_{-0.6}^{+0.6}$&$-6.5_{-0.6}^{+0.6}$&$-8.5_{-3.7}^{+2.0}$&$-6.3_{-0.6}^{+0.7}$&$-6.6_{-0.6}^{+0.5}$&$-6.6_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CO})$&-6.903&$-10.5_{-2.7}^{+3.1}$&$-7.8_{-4.4}^{+4.4}$&$-8.0_{-4.3}^{+4.5}$&$-8.2_{-4.2}^{+4.7}$&$-8.1_{-3.9}^{+4.0}$&$-7.5_{-4.5}^{+4.3}$&$-7.9_{-4.5}^{+4.7}$&$-7.9_{-4.4}^{+4.6}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-10.5_{-2.6}^{+2.7}$&$-8.8_{-3.6}^{+3.8}$&$-8.5_{-3.8}^{+3.7}$&$-8.9_{-3.8}^{+3.5}$&$-9.6_{-3.1}^{+3.5}$&$-8.9_{-3.9}^{+4.0}$&$-9.2_{-3.6}^{+3.8}$&$-9.3_{-3.5}^{+3.6}$\\ 
\hline
\multicolumn{10}{c}{} \\

\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$17.4_{-8.8}^{+12.5}$&$16.5_{-8.9}^{+14.5}$&$14.4_{-6.6}^{+9.1}$&$14.4_{-6.5}^{+12.1}$&$14.5_{-7.4}^{+12.9}$&$13.5_{-6.0}^{+9.5}$&$14.9_{-6.1}^{+10.7}$&$19.8_{-8.1}^{+13.1}$\\ 

$a_2$&99.70&$77.0_{-39.5}^{+54.3}$&$62.6_{-29.8}^{+56.0}$&$63.4_{-26.0}^{+39.7}$&$60.2_{-21.5}^{+32.0}$&$61.2_{-29.6}^{+44.3}$&$59.6_{-23.1}^{+37.7}$&$67.2_{-24.4}^{+32.6}$&$86.9_{-27.1}^{+35.4}$\\ 

$a_1$&146.63&$127.5_{-56.3}^{+93.3}$&$100.0_{-38.0}^{+78.3}$&$109.7_{-44.5}^{+85.1}$&$90.2_{-29.3}^{+46.2}$&$105.6_{-40.4}^{+68.9}$&$109.0_{-51.3}^{+61.0}$&$107.0_{-43.6}^{+60.5}$&$135.3_{-43.5}^{+47.2}$\\ 

$a_0$&285.22&$286.7_{-47.0}^{+57.0}$&$280.9_{-30.5}^{+39.3}$&$286.4_{-35.9}^{+58.7}$&$264.2_{-20.0}^{+30.3}$&$287.3_{-37.2}^{+46.9}$&$286.0_{-41.4}^{+41.3}$&$276.4_{-30.8}^{+38.4}$&$284.5_{-26.5}^{+31.4}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.0_{-0.3}^{+0.4}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.4}^{+0.4}$&$0.2_{-0.3}^{+0.2}$&$-0.0_{-0.3}^{+0.4}$&$-0.0_{-0.3}^{+0.5}$&$0.1_{-0.3}^{+0.4}$&$0.0_{-0.2}^{+0.2}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$1.0_{-0.1}^{+0.1}$&$1.02_{-0.07}^{+0.07}$&$1.03_{-0.05}^{+0.05}$&$1.02_{-0.04}^{+0.04}$&$1.00_{-0.08}^{+0.08}$&$1.03_{-0.05}^{+0.05}$&$1.01_{-0.04}^{+0.04}$&$1.00_{-0.03}^{+0.03}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.1_{-4.5}^{+4.3}$&$-7.5_{-4.7}^{+4.6}$&$-7.4_{-4.6}^{+4.5}$&$-7.5_{-4.7}^{+4.6}$&$-7.5_{-4.7}^{+4.7}$&$-7.4_{-4.6}^{+4.5}$&$-7.5_{-4.7}^{+4.5}$&$-7.6_{-4.5}^{+4.8}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.6_{-4.3}^{+4.4}$&$-7.8_{-4.2}^{+4.6}$&$-7.5_{-4.6}^{+4.5}$&$-7.4_{-4.9}^{+4.7}$&$-7.5_{-4.5}^{+4.6}$&$-7.2_{-4.7}^{+4.4}$&$-7.5_{-4.5}^{+4.7}$&$-7.9_{-4.6}^{+4.9}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-3.1_{-1.1}^{+1.0}$&$-2.8_{-0.8}^{+0.7}$&$-2.6_{-0.8}^{+0.8}$&$-3.1_{-0.6}^{+0.6}$&$-2.8_{-0.9}^{+0.9}$&$-2.7_{-0.9}^{+0.7}$&$-3.0_{-0.7}^{+0.6}$&$-2.9_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-3.7_{-0.9}^{+0.9}$&$-3.3_{-0.7}^{+0.7}$&$-3.1_{-0.7}^{+0.8}$&$-3.6_{-0.5}^{+0.6}$&$-3.3_{-0.8}^{+0.8}$&$-3.2_{-0.8}^{+0.6}$&$-3.4_{-0.6}^{+0.5}$&$-3.3_{-0.5}^{+0.4}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-8.8_{-3.5}^{+3.0}$&$-9.3_{-3.5}^{+3.1}$&$-7.9_{-4.2}^{+2.3}$&$-6.9_{-4.3}^{+1.1}$&$-9.2_{-3.4}^{+3.2}$&$-7.9_{-4.2}^{+2.3}$&$-6.3_{-2.0}^{+0.9}$&$-5.8_{-0.6}^{+0.6}$\\ 

$L(\mathrm{O_3})$&-6.523&$-7.2_{-4.3}^{+1.1}$&$-6.5_{-0.5}^{+0.5}$&$-6.4_{-0.6}^{+0.6}$&$-6.7_{-0.4}^{+0.4}$&$-6.5_{-0.7}^{+0.7}$&$-6.5_{-0.6}^{+0.5}$&$-6.6_{-0.5}^{+0.4}$&$-6.5_{-0.4}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.6_{-4.2}^{+4.4}$&$-7.5_{-4.6}^{+4.5}$&$-8.0_{-4.4}^{+4.8}$&$-7.9_{-4.3}^{+4.6}$&$-7.7_{-4.3}^{+4.5}$&$-7.8_{-4.5}^{+4.4}$&$-8.0_{-4.3}^{+4.4}$&$-8.3_{-4.2}^{+4.3}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-8.3_{-3.7}^{+3.8}$&$-8.9_{-3.6}^{+3.9}$&$-8.6_{-3.8}^{+3.5}$&$-9.0_{-3.7}^{+3.2}$&$-8.5_{-4.0}^{+4.0}$&$-8.8_{-3.6}^{+3.6}$&$-9.2_{-3.6}^{+3.3}$&$-9.4_{-3.4}^{+3.3}$\\ 
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}





\begin{table*}
\caption{Retrieval results for the $4-18.5\,\mu$m wavelength range for the optimized case.}             % title of Table
\label{table:4-18.5_opt}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.2_{-0.2}^{+0.3}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$22.6_{-11.5}^{+18.3}$&$13.1_{-6.3}^{+9.8}$&$13.0_{-6.1}^{+7.8}$&$11.7_{-5.6}^{+8.5}$&$16.4_{-8.0}^{+15.1}$&$10.8_{-5.4}^{+9.2}$&$12.2_{-5.8}^{+10.8}$&$12.1_{-5.4}^{+11.2}$\\ 

$a_2$&99.70&$101.3_{-42.6}^{+51.4}$&$61.5_{-31.9}^{+42.6}$&$51.7_{-26.4}^{+34.6}$&$49.0_{-25.0}^{+32.9}$&$71.5_{-34.7}^{+49.6}$&$39.5_{-20.3}^{+29.5}$&$55.6_{-27.4}^{+43.9}$&$47.8_{-20.3}^{+39.1}$\\ 

$a_1$&146.63&$135.8_{-56.7}^{+57.9}$&$132.1_{-47.6}^{+62.6}$&$94.7_{-39.4}^{+71.5}$&$94.7_{-32.5}^{+61.3}$&$113.8_{-44.9}^{+53.7}$&$65.7_{-23.4}^{+36.2}$&$112.4_{-45.4}^{+81.2}$&$89.8_{-40.3}^{+47.5}$\\ 

$a_0$&285.22&$211.1_{-79.7}^{+60.6}$&$304.6_{-36.4}^{+45.6}$&$283.3_{-37.6}^{+55.6}$&$290.9_{-28.4}^{+48.1}$&$246.6_{-67.9}^{+56.3}$&$259.4_{-28.2}^{+30.6}$&$310.0_{-44.4}^{+55.4}$&$275.8_{-28.1}^{+29.8}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.5_{-0.3}^{+0.3}$&$-0.1_{-0.3}^{+0.3}$&$0.1_{-0.4}^{+0.5}$&$-0.0_{-0.4}^{+0.3}$&$0.4_{-0.4}^{+0.3}$&$0.4_{-0.4}^{+0.3}$&$-0.2_{-0.4}^{+0.5}$&$0.1_{-0.3}^{+0.4}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.9_{-0.1}^{+0.1}$&$0.98_{-0.09}^{+0.09}$&$0.99_{-0.07}^{+0.07}$&$1.01_{-0.05}^{+0.06}$&$0.9_{-0.1}^{+0.1}$&$1.00_{-0.08}^{+0.07}$&$1.01_{-0.05}^{+0.05}$&$1.01_{-0.04}^{+0.04}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-6.6_{-4.4}^{+4.0}$&$-7.2_{-4.6}^{+4.1}$&$-7.0_{-4.6}^{+4.1}$&$-7.1_{-4.7}^{+4.3}$&$-8.0_{-4.1}^{+4.3}$&$-7.8_{-4.4}^{+4.6}$&$-7.8_{-4.4}^{+4.7}$&$-7.6_{-4.6}^{+4.6}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.3_{-4.4}^{+4.4}$&$-7.8_{-4.4}^{+4.4}$&$-7.9_{-4.2}^{+4.5}$&$-7.3_{-4.5}^{+4.3}$&$-7.7_{-4.5}^{+4.6}$&$-7.3_{-4.5}^{+4.2}$&$-7.5_{-4.5}^{+4.5}$&$-7.3_{-4.8}^{+4.6}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-3.9_{-1.4}^{+0.9}$&$-2.1_{-0.9}^{+0.9}$&$-2.5_{-0.9}^{+1.1}$&$-2.2_{-0.8}^{+0.8}$&$-3.3_{-0.8}^{+1.1}$&$-3.1_{-0.8}^{+0.9}$&$-2.0_{-0.9}^{+0.9}$&$-2.7_{-0.8}^{+0.7}$\\

$L(\mathrm{CO_2})$&-3.387&$-6.3_{-4.3}^{+1.9}$&$-3.5_{-1.1}^{+1.0}$&$-3.5_{-0.8}^{+1.0}$&$-3.1_{-0.8}^{+0.7}$&$-5.0_{-3.1}^{+1.4}$&$-3.9_{-0.8}^{+0.9}$&$-2.8_{-0.9}^{+0.8}$&$-3.4_{-0.7}^{+0.7}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.6_{-3.1}^{+2.8}$&$-9.5_{-3.2}^{+3.3}$&$-9.4_{-3.4}^{+3.0}$&$-8.8_{-3.7}^{+2.9}$&$-10.1_{-2.9}^{+2.9}$&$-9.9_{-3.1}^{+3.0}$&$-7.8_{-4.4}^{+2.5}$&$-6.7_{-3.9}^{+1.1}$\\ 

$L(\mathrm{O_3})$&-6.523&$-9.7_{-3.1}^{+2.4}$&$-6.2_{-0.7}^{+0.7}$&$-6.5_{-0.6}^{+0.7}$&$-6.2_{-0.6}^{+0.6}$&$-7.2_{-2.1}^{+0.9}$&$-6.8_{-0.6}^{+0.6}$&$-6.0_{-0.7}^{+0.7}$&$-6.5_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CO})$&-6.903&$-8.9_{-3.6}^{+3.9}$&$-7.8_{-4.5}^{+4.6}$&$-7.2_{-4.4}^{+4.3}$&$-7.7_{-4.5}^{+4.3}$&$-8.2_{-4.1}^{+4.5}$&$-8.1_{-4.3}^{+4.7}$&$-7.8_{-4.5}^{+4.6}$&$-8.0_{-4.3}^{+4.3}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.7_{-3.1}^{+3.5}$&$-8.2_{-4.0}^{+3.8}$&$-8.4_{-3.8}^{+3.7}$&$-8.5_{-3.8}^{+3.6}$&$-8.7_{-3.5}^{+3.6}$&$-8.9_{-3.6}^{+3.4}$&$-9.3_{-3.5}^{+3.7}$&$-9.2_{-3.4}^{+3.2}$\\ 
\hline
\multicolumn{10}{c}{} \\

\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$13.1_{-6.5}^{+10.4}$&$11.5_{-5.5}^{+7.8}$&$13.9_{-5.8}^{+10.5}$&$15.7_{-6.7}^{+13.0}$&$13.2_{-6.3}^{+9.8}$&$17.0_{-7.5}^{+13.7}$&$16.3_{-7.2}^{+13.5}$&$19.7_{-8.7}^{+14.4}$\\ 

$a_2$&99.70&$59.2_{-31.6}^{+44.2}$&$36.8_{-17.5}^{+22.5}$&$62.0_{-25.8}^{+42.8}$&$74.7_{-28.0}^{+44.0}$&$53.6_{-26.3}^{+36.4}$&$81.4_{-35.6}^{+57.7}$&$73.6_{-27.1}^{+41.0}$&$84.6_{-27.7}^{+40.5}$\\ 

$a_1$&146.63&$125.9_{-51.9}^{+69.8}$&$60.8_{-20.1}^{+29.0}$&$113.3_{-41.9}^{+92.3}$&$130.1_{-48.3}^{+68.4}$&$97.0_{-33.6}^{+55.4}$&$156.6_{-70.0}^{+101.0}$&$118.9_{-43.0}^{+62.2}$&$132.7_{-47.1}^{+51.0}$\\ 

$a_0$&285.22&$298.7_{-49.8}^{+56.7}$&$257.1_{-20.7}^{+24.7}$&$299.9_{-37.3}^{+63.9}$&$298.7_{-37.0}^{+40.7}$&$280.5_{-31.4}^{+41.7}$&$325.9_{-53.1}^{+71.9}$&$282.2_{-28.6}^{+43.2}$&$283.1_{-27.3}^{+31.3}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$-0.1_{-0.4}^{+0.4}$&$0.4_{-0.3}^{+0.3}$&$-0.1_{-0.4}^{+0.4}$&$-0.1_{-0.2}^{+0.3}$&$0.1_{-0.3}^{+0.3}$&$-0.3_{-0.3}^{+0.4}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.2}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$1.0_{-0.1}^{+0.1}$&$1.01_{-0.06}^{+0.07}$&$1.01_{-0.05}^{+0.05}$&$1.00_{-0.03}^{+0.04}$&$1.00_{-0.08}^{+0.08}$&$1.01_{-0.05}^{+0.05}$&$1.00_{-0.03}^{+0.03}$&$1.00_{-0.02}^{+0.02}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.6_{-4.2}^{+4.3}$&$-7.6_{-4.3}^{+4.5}$&$-7.3_{-4.3}^{+4.3}$&$-7.5_{-4.6}^{+4.6}$&$-7.9_{-4.4}^{+4.7}$&$-7.6_{-4.8}^{+4.6}$&$-7.5_{-4.4}^{+4.6}$&$-7.4_{-4.6}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.7_{-4.3}^{+4.5}$&$-7.4_{-4.6}^{+4.4}$&$-7.4_{-4.6}^{+4.5}$&$-7.2_{-4.7}^{+4.4}$&$-7.1_{-4.7}^{+4.3}$&$-8.1_{-4.3}^{+4.9}$&$-7.4_{-4.7}^{+4.5}$&$-7.8_{-4.7}^{+4.9}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-2.4_{-1.1}^{+1.0}$&$-3.1_{-0.7}^{+0.8}$&$-2.3_{-0.9}^{+0.8}$&$-2.7_{-0.7}^{+0.6}$&$-2.6_{-0.8}^{+0.8}$&$-2.2_{-0.8}^{+0.8}$&$-2.9_{-0.6}^{+0.6}$&$-3.0_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-3.6_{-1.3}^{+1.1}$&$-3.8_{-0.6}^{+0.7}$&$-3.0_{-0.7}^{+0.8}$&$-3.1_{-0.6}^{+0.5}$&$-3.5_{-0.8}^{+0.8}$&$-2.8_{-0.7}^{+0.7}$&$-3.3_{-0.6}^{+0.6}$&$-3.4_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.9_{-3.1}^{+3.2}$&$-9.1_{-3.7}^{+2.6}$&$-6.2_{-3.9}^{+1.2}$&$-5.7_{-0.7}^{+0.6}$&$-8.4_{-3.8}^{+2.5}$&$-5.5_{-1.1}^{+0.9}$&$-5.8_{-0.6}^{+0.6}$&$-5.8_{-0.5}^{+0.5}$\\ 

$L(\mathrm{O_3})$&-6.523&$-6.4_{-1.0}^{+0.8}$&$-6.8_{-0.5}^{+0.5}$&$-6.2_{-0.6}^{+0.6}$&$-6.3_{-0.5}^{+0.4}$&$-6.5_{-0.6}^{+0.6}$&$-6.1_{-0.5}^{+0.6}$&$-6.5_{-0.4}^{+0.5}$&$-6.5_{-0.4}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-8.2_{-3.9}^{+4.5}$&$-8.0_{-4.2}^{+4.6}$&$-8.0_{-4.4}^{+4.5}$&$-8.3_{-4.1}^{+4.6}$&$-7.4_{-4.4}^{+4.6}$&$-7.8_{-4.5}^{+4.3}$&$-7.9_{-4.4}^{+4.3}$&$-8.7_{-4.0}^{+4.2}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-8.5_{-3.9}^{+3.9}$&$-9.2_{-3.3}^{+3.4}$&$-9.0_{-3.5}^{+3.5}$&$-9.3_{-3.5}^{+3.2}$&$-8.7_{-3.7}^{+3.7}$&$-9.0_{-3.7}^{+3.7}$&$-9.5_{-3.4}^{+3.2}$&$-9.9_{-3.2}^{+3.1}$\\ 
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}


















\begin{table*}
\caption{Retrieval results for the $6-17\,\mu$m wavelength range for the nominal case.}           % title of Table
\label{table:6-17}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.2_{-0.3}^{+0.3}$&$1.2_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.2_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$43.0_{-23.8}^{+29.6}$&$30.0_{-17.0}^{+29.9}$&$17.9_{-9.1}^{+17.6}$&$15.4_{-7.3}^{+11.3}$&$35.5_{-18.3}^{+26.6}$&$15.5_{-7.5}^{+11.6}$&$16.8_{-8.7}^{+16.3}$&$16.8_{-7.8}^{+14.4}$\\ 

$a_2$&99.70&$167.4_{-77.4}^{+96.9}$&$120.6_{-62.6}^{+96.3}$&$71.6_{-33.6}^{+50.3}$&$59.6_{-25.6}^{+31.5}$&$130.7_{-62.0}^{+97.7}$&$63.4_{-27.9}^{+34.7}$&$61.4_{-28.2}^{+57.6}$&$63.7_{-26.0}^{+41.9}$\\ 

$a_1$&146.63&$148.2_{-79.8}^{+122.3}$&$118.5_{-47.4}^{+71.1}$&$101.1_{-37.0}^{+59.8}$&$80.6_{-28.1}^{+41.1}$&$103.7_{-54.7}^{+117.6}$&$96.6_{-32.6}^{+40.7}$&$84.1_{-34.6}^{+81.8}$&$86.8_{-38.3}^{+55.1}$\\ 

$a_0$&285.22&$217.6_{-88.8}^{+92.3}$&$235.7_{-70.0}^{+47.4}$&$269.6_{-34.3}^{+37.1}$&$258.0_{-26.5}^{+26.7}$&$213.8_{-61.3}^{+53.4}$&$269.6_{-32.5}^{+35.4}$&$261.2_{-27.0}^{+45.5}$&$258.2_{-22.8}^{+29.4}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.4_{-0.4}^{+0.3}$&$0.3_{-0.3}^{+0.2}$&$0.2_{-0.3}^{+0.3}$&$0.3_{-0.3}^{+0.2}$&$0.5_{-0.3}^{+0.2}$&$0.2_{-0.3}^{+0.3}$&$0.2_{-0.4}^{+0.3}$&$0.3_{-0.3}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.9_{-0.1}^{+0.1}$&$1.01_{-0.09}^{+0.1}$&$1.00_{-0.08}^{+0.09}$&$1.01_{-0.07}^{+0.07}$&$0.9_{-0.1}^{+0.1}$&$0.99_{-0.08}^{+0.09}$&$1.01_{-0.07}^{+0.07}$&$1.01_{-0.06}^{+0.06}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.5_{-4.3}^{+4.2}$&$-7.4_{-4.4}^{+4.3}$&$-7.4_{-4.5}^{+4.4}$&$-7.5_{-4.6}^{+4.8}$&$-8.1_{-4.1}^{+4.4}$&$-7.6_{-4.3}^{+4.7}$&$-7.1_{-4.8}^{+4.4}$&$-7.6_{-4.8}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.7_{-4.1}^{+4.5}$&$-7.5_{-4.1}^{+4.4}$&$-7.2_{-4.5}^{+4.4}$&$-7.8_{-4.7}^{+4.8}$&$-6.8_{-4.9}^{+4.2}$&$-7.3_{-4.5}^{+4.4}$&$-7.7_{-4.6}^{+4.7}$&$-7.6_{-4.6}^{+4.7}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-9.5_{-3.1}^{+3.3}$&$-5.5_{-5.1}^{+2.2}$&$-3.2_{-1.1}^{+0.9}$&$-3.2_{-0.8}^{+0.8}$&$-8.6_{-3.6}^{+3.4}$&$-3.2_{-1.2}^{+1.0}$&$-3.2_{-0.8}^{+0.9}$&$-3.2_{-0.7}^{+0.7}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-5.1_{-2.2}^{+1.0}$&$-4.0_{-0.5}^{+0.6}$&$-3.6_{-0.6}^{+0.7}$&$-3.8_{-0.6}^{+0.6}$&$-4.5_{-0.7}^{+0.6}$&$-3.6_{-0.7}^{+0.8}$&$-3.7_{-0.7}^{+0.7}$&$-3.8_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.6_{-3.1}^{+2.8}$&$-9.1_{-3.5}^{+3.1}$&$-8.4_{-3.6}^{+2.8}$&$-9.3_{-3.5}^{+3.0}$&$-9.6_{-3.2}^{+3.1}$&$-8.9_{-3.9}^{+3.2}$&$-9.2_{-3.5}^{+3.0}$&$-9.2_{-3.5}^{+2.9}$\\ 

$L(\mathrm{O_3})$&-6.523&$-10.4_{-2.7}^{+2.7}$&$-7.8_{-3.5}^{+1.1}$&$-6.7_{-0.6}^{+0.6}$&$-6.8_{-0.5}^{+0.5}$&$-9.6_{-3.1}^{+2.3}$&$-6.7_{-0.7}^{+0.7}$&$-6.8_{-0.5}^{+0.6}$&$-6.8_{-0.4}^{+0.5}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.8_{-4.1}^{+4.4}$&$-7.1_{-4.4}^{+4.5}$&$-7.8_{-4.3}^{+4.4}$&$-7.4_{-4.8}^{+4.7}$&$-7.7_{-4.2}^{+4.4}$&$-7.4_{-4.4}^{+4.4}$&$-7.6_{-4.8}^{+4.7}$&$-7.4_{-4.7}^{+4.7}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.7_{-3.0}^{+3.0}$&$-9.4_{-3.3}^{+3.3}$&$-8.9_{-3.7}^{+3.9}$&$-8.5_{-4.0}^{+3.6}$&$-10.0_{-2.9}^{+2.9}$&$-8.7_{-3.7}^{+3.8}$&$-9.0_{-3.8}^{+3.7}$&$-8.9_{-3.7}^{+3.6}$\\
\hline
\multicolumn{10}{c}{} \\

\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.2_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$33.5_{-17.3}^{+22.8}$&$15.0_{-7.6}^{+14.3}$&$16.3_{-7.8}^{+13.6}$&$15.5_{-6.6}^{+12.2}$&$17.8_{-9.1}^{+18.9}$&$16.2_{-7.7}^{+13.6}$&$19.0_{-8.5}^{+16.5}$&$19.4_{-8.7}^{+15.5}$\\ 

$a_2$&99.70&$127.0_{-57.5}^{+75.9}$&$62.9_{-28.5}^{+39.9}$&$63.1_{-28.5}^{+48.4}$&$66.3_{-24.3}^{+30.7}$&$70.1_{-31.0}^{+43.5}$&$67.0_{-26.8}^{+35.9}$&$78.3_{-26.8}^{+52.3}$&$81.7_{-30.0}^{+48.2}$\\ 

$a_1$&146.63&$118.8_{-58.6}^{+109.9}$&$94.5_{-31.0}^{+47.3}$&$92.7_{-48.3}^{+82.6}$&$92.8_{-33.7}^{+50.9}$&$102.3_{-35.8}^{+45.1}$&$98.4_{-39.0}^{+56.9}$&$126.9_{-54.5}^{+60.6}$&$119.9_{-50.9}^{+72.1}$\\ 

$a_0$&285.22&$232.6_{-50.4}^{+49.7}$&$271.5_{-30.5}^{+34.5}$&$266.7_{-32.9}^{+48.3}$&$261.4_{-22.0}^{+32.4}$&$269.0_{-32.6}^{+37.2}$&$271.0_{-29.7}^{+36.1}$&$281.0_{-32.5}^{+35.3}$&$275.9_{-30.8}^{+43.7}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.3_{-0.3}^{+0.2}$&$0.1_{-0.3}^{+0.3}$&$0.2_{-0.4}^{+0.5}$&$0.2_{-0.3}^{+0.3}$&$0.1_{-0.3}^{+0.3}$&$0.1_{-0.3}^{+0.3}$&$0.0_{-0.2}^{+0.3}$&$0.1_{-0.3}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$1.0_{-0.1}^{+0.1}$&$1.01_{-0.08}^{+0.08}$&$1.01_{-0.06}^{+0.06}$&$1.02_{-0.05}^{+0.05}$&$1.0_{-0.1}^{+0.1}$&$1.01_{-0.06}^{+0.07}$&$1.02_{-0.05}^{+0.05}$&$1.01_{-0.04}^{+0.04}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-8.0_{-4.1}^{+4.5}$&$-7.4_{-4.8}^{+4.6}$&$-7.6_{-4.5}^{+4.7}$&$-7.5_{-4.6}^{+4.6}$&$-7.4_{-4.4}^{+4.3}$&$-7.3_{-4.7}^{+4.5}$&$-7.7_{-4.7}^{+4.9}$&$-7.4_{-4.7}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.3_{-4.4}^{+4.4}$&$-7.4_{-4.5}^{+4.4}$&$-7.6_{-4.6}^{+4.6}$&$-7.7_{-4.7}^{+4.9}$&$-7.4_{-4.6}^{+4.5}$&$-7.7_{-4.5}^{+4.7}$&$-7.3_{-4.6}^{+4.5}$&$-7.5_{-4.6}^{+4.8}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-7.5_{-4.5}^{+3.2}$&$-3.0_{-0.9}^{+0.9}$&$-3.1_{-0.9}^{+0.8}$&$-3.2_{-0.6}^{+0.7}$&$-3.5_{-1.6}^{+1.1}$&$-3.0_{-0.7}^{+0.7}$&$-2.9_{-0.6}^{+0.6}$&$-3.0_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-4.1_{-0.6}^{+0.6}$&$-3.5_{-0.7}^{+0.7}$&$-3.6_{-0.8}^{+0.7}$&$-3.6_{-0.6}^{+0.6}$&$-3.6_{-0.6}^{+0.7}$&$-3.5_{-0.6}^{+0.7}$&$-3.4_{-0.6}^{+0.5}$&$-3.5_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-8.8_{-3.5}^{+2.9}$&$-9.1_{-3.6}^{+3.1}$&$-9.3_{-3.5}^{+3.1}$&$-8.2_{-3.9}^{+2.2}$&$-9.0_{-3.5}^{+3.1}$&$-8.4_{-4.1}^{+2.5}$&$-7.1_{-4.5}^{+1.4}$&$-6.3_{-2.6}^{+0.9}$\\ 

$L(\mathrm{O_3})$&-6.523&$-8.4_{-3.7}^{+1.5}$&$-6.6_{-0.5}^{+0.6}$&$-6.7_{-0.6}^{+0.6}$&$-6.7_{-0.5}^{+0.5}$&$-6.8_{-1.3}^{+0.7}$&$-6.6_{-0.5}^{+0.5}$&$-6.6_{-0.4}^{+0.5}$&$-6.6_{-0.5}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-8.0_{-4.1}^{+4.7}$&$-7.4_{-4.7}^{+4.5}$&$-7.4_{-4.7}^{+4.5}$&$-7.9_{-4.4}^{+4.6}$&$-7.2_{-4.5}^{+4.4}$&$-7.7_{-4.6}^{+4.8}$&$-7.2_{-4.6}^{+4.4}$&$-7.2_{-4.8}^{+4.5}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-9.5_{-3.1}^{+3.0}$&$-8.9_{-3.8}^{+3.9}$&$-8.8_{-3.6}^{+3.8}$&$-9.3_{-3.5}^{+3.6}$&$-8.5_{-3.8}^{+3.5}$&$-8.5_{-3.9}^{+3.6}$&$-9.2_{-3.6}^{+3.8}$&$-9.3_{-3.6}^{+3.6}$\\ 
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}





\begin{table*}
\caption{Retrieval results for the $6-17\,\mu$m wavelength range for the optimized case.}           % title of Table
\label{table:6-17_opt}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{lc|cccc|cccc}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=20}&\multicolumn{4}{c}{R=35}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.3_{-0.3}^{+0.3}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$32.1_{-16.6}^{+27.0}$&$14.7_{-7.7}^{+11.3}$&$11.4_{-5.5}^{+8.5}$&$12.6_{-5.9}^{+9.3}$&$18.4_{-9.5}^{+12.0}$&$13.3_{-6.7}^{+10.0}$&$12.2_{-5.9}^{+10.3}$&$14.3_{-6.9}^{+10.4}$\\ 

$a_2$&99.70&$113.7_{-48.6}^{+76.8}$&$64.6_{-35.0}^{+43.4}$&$46.9_{-23.7}^{+33.7}$&$54.6_{-26.9}^{+38.5}$&$80.2_{-36.5}^{+41.0}$&$55.2_{-28.9}^{+32.8}$&$49.5_{-22.9}^{+32.5}$&$54.5_{-23.4}^{+37.8}$\\ 

$a_1$&146.63&$114.4_{-57.1}^{+79.8}$&$114.1_{-44.2}^{+71.8}$&$87.6_{-31.7}^{+55.1}$&$110.4_{-37.0}^{+63.1}$&$125.6_{-51.4}^{+64.4}$&$97.7_{-36.3}^{+55.9}$&$91.4_{-36.8}^{+48.6}$&$88.7_{-31.1}^{+65.9}$\\ 

$a_0$&285.22&$194.6_{-72.8}^{+68.0}$&$277.5_{-44.3}^{+53.6}$&$276.4_{-30.8}^{+46.8}$&$310.2_{-35.3}^{+46.0}$&$247.1_{-59.5}^{+47.8}$&$281.9_{-34.2}^{+44.8}$&$283.4_{-31.7}^{+38.2}$&$277.0_{-26.1}^{+42.8}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.5_{-0.4}^{+0.3}$&$0.1_{-0.4}^{+0.3}$&$0.2_{-0.4}^{+0.3}$&$-0.2_{-0.3}^{+0.4}$&$0.3_{-0.3}^{+0.3}$&$0.1_{-0.4}^{+0.3}$&$0.1_{-0.3}^{+0.4}$&$0.1_{-0.4}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$1.0_{-0.1}^{+0.1}$&$0.96_{-0.09}^{+0.1}$&$0.99_{-0.08}^{+0.07}$&$0.99_{-0.06}^{+0.06}$&$0.9_{-0.1}^{+0.1}$&$0.98_{-0.08}^{+0.08}$&$1.00_{-0.06}^{+0.06}$&$1.00_{-0.05}^{+0.04}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.1_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.7_{-4.2}^{+4.2}$&$-7.4_{-4.4}^{+4.5}$&$-7.4_{-4.6}^{+4.4}$&$-7.5_{-4.7}^{+4.4}$&$-7.4_{-4.4}^{+4.5}$&$-7.2_{-4.6}^{+4.4}$&$-7.8_{-4.7}^{+4.7}$&$-7.4_{-4.6}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.0_{-4.6}^{+4.8}$&$-7.5_{-4.4}^{+4.4}$&$-7.4_{-4.5}^{+4.4}$&$-7.9_{-4.3}^{+4.5}$&$-6.7_{-4.8}^{+4.3}$&$-7.4_{-4.5}^{+4.6}$&$-7.8_{-4.5}^{+4.7}$&$-7.6_{-4.5}^{+4.5}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-5.1_{-5.5}^{+1.5}$&$-2.7_{-0.9}^{+1.0}$&$-2.6_{-0.8}^{+1.0}$&$-1.9_{-0.8}^{+0.8}$&$-3.3_{-1.0}^{+0.9}$&$-2.4_{-0.9}^{+0.8}$&$-2.5_{-0.8}^{+0.8}$&$-2.6_{-0.7}^{+0.8}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-5.6_{-3.0}^{+1.5}$&$-4.0_{-1.1}^{+1.0}$&$-3.7_{-0.8}^{+0.9}$&$-3.0_{-0.8}^{+0.7}$&$-4.8_{-2.0}^{+1.2}$&$-3.5_{-0.8}^{+0.8}$&$-3.4_{-0.7}^{+0.8}$&$-3.4_{-0.7}^{+0.7}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-9.9_{-2.9}^{+2.7}$&$-9.9_{-2.9}^{+3.1}$&$-9.5_{-3.4}^{+2.9}$&$-9.0_{-3.6}^{+3.1}$&$-9.6_{-3.0}^{+2.8}$&$-9.5_{-3.4}^{+3.0}$&$-9.1_{-3.5}^{+2.8}$&$-7.2_{-4.2}^{+1.4}$\\ 

$L(\mathrm{O_3})$&-6.523&$-10.6_{-2.6}^{+2.7}$&$-6.6_{-0.7}^{+0.7}$&$-6.5_{-0.6}^{+0.6}$&$-6.0_{-0.6}^{+0.6}$&$-7.2_{-3.1}^{+0.8}$&$-6.4_{-0.6}^{+0.6}$&$-6.4_{-0.6}^{+0.6}$&$-6.5_{-0.5}^{+0.5}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.5_{-4.3}^{+4.3}$&$-7.2_{-4.5}^{+4.2}$&$-7.2_{-4.7}^{+4.3}$&$-7.5_{-4.5}^{+4.3}$&$-6.7_{-4.6}^{+4.0}$&$-7.5_{-4.6}^{+4.6}$&$-7.5_{-4.7}^{+4.4}$&$-7.8_{-4.5}^{+4.7}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-10.1_{-2.8}^{+3.1}$&$-8.7_{-3.8}^{+4.0}$&$-8.9_{-3.7}^{+3.8}$&$-8.7_{-3.7}^{+3.7}$&$-8.7_{-3.6}^{+3.6}$&$-8.9_{-3.8}^{+3.8}$&$-9.1_{-3.6}^{+3.5}$&$-9.4_{-3.4}^{+3.4}$\\ 
\hline
\multicolumn{10}{c}{} \\

\hline\hline                 % inserts double horizontal lines
&&\multicolumn{4}{c|}{R=50}&\multicolumn{4}{c}{R=100}\\
Parameter&Input&S/N=5&S/N=10&S/N=15&S/N=20&S/N=5&S/N=10&S/N=15&S/N=20\\
\hline
$\sqrt[4]{a_4}$&1.14&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.0_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$&$1.1_{-0.2}^{+0.2}$\\ 

$a_3$&23.12&$16.4_{-8.1}^{+13.3}$&$14.0_{-7.1}^{+10.3}$&$13.0_{-6.5}^{+12.7}$&$14.9_{-6.8}^{+11.3}$&$12.5_{-6.0}^{+10.9}$&$15.0_{-7.5}^{+11.7}$&$19.4_{-8.9}^{+18.3}$&$21.8_{-9.8}^{+16.8}$\\ 

$a_2$&99.70&$76.1_{-37.6}^{+42.9}$&$57.8_{-31.1}^{+43.0}$&$49.6_{-23.1}^{+40.7}$&$67.8_{-30.5}^{+36.7}$&$56.3_{-28.2}^{+38.3}$&$68.5_{-33.7}^{+53.1}$&$88.9_{-37.4}^{+66.8}$&$93.1_{-32.7}^{+56.3}$\\ 

$a_1$&146.63&$130.4_{-49.4}^{+65.2}$&$105.9_{-43.8}^{+77.0}$&$84.5_{-32.7}^{+56.4}$&$119.0_{-59.8}^{+60.0}$&$99.9_{-37.2}^{+66.8}$&$126.8_{-59.3}^{+106.8}$&$161.8_{-83.2}^{+94.6}$&$149.2_{-59.5}^{+80.3}$\\ 

$a_0$&285.22&$268.3_{-45.0}^{+44.3}$&$293.2_{-34.0}^{+53.4}$&$274.2_{-27.1}^{+35.7}$&$286.0_{-37.7}^{+47.4}$&$277.1_{-33.1}^{+47.8}$&$308.5_{-51.4}^{+68.5}$&$307.7_{-51.1}^{+59.3}$&$295.9_{-37.8}^{+49.0}$\\ 

\cdashline{1-10}$L\left(P_0\left[\mathrm{bar}\right]\right)$&0.006&$0.2_{-0.3}^{+0.3}$&$-0.0_{-0.4}^{+0.4}$&$0.1_{-0.3}^{+0.4}$&$0.0_{-0.3}^{+0.4}$&$0.1_{-0.4}^{+0.3}$&$-0.2_{-0.4}^{+0.5}$&$-0.1_{-0.3}^{+0.4}$&$-0.1_{-0.3}^{+0.3}$\\ 

$R\,\left[R_\oplus\right]$&1.0&$0.9_{-0.1}^{+0.1}$&$0.99_{-0.07}^{+0.07}$&$1.00_{-0.05}^{+0.05}$&$1.00_{-0.04}^{+0.04}$&$0.99_{-0.09}^{+0.09}$&$1.00_{-0.05}^{+0.06}$&$1.00_{-0.03}^{+0.03}$&$1.00_{-0.03}^{+0.03}$\\ 

$L\left(M\,\left[M_\oplus\right]\right)$&0.0&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$-0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$&$0.0_{-0.3}^{+0.3}$\\ 

\cdashline{1-10}$L(\mathrm{N_2})$&-0.107&$-7.6_{-4.2}^{+4.5}$&$-7.2_{-4.7}^{+4.4}$&$-7.6_{-4.7}^{+4.7}$&$-7.6_{-4.6}^{+4.6}$&$-7.8_{-4.1}^{+4.5}$&$-7.4_{-4.6}^{+4.6}$&$-7.7_{-4.5}^{+4.9}$&$-7.5_{-4.5}^{+4.7}$\\ 

$L(\mathrm{O_2})$&-0.679&$-7.7_{-4.3}^{+4.6}$&$-7.3_{-4.5}^{+4.4}$&$-7.4_{-4.8}^{+4.6}$&$-7.3_{-4.6}^{+4.5}$&$-7.5_{-4.5}^{+4.5}$&$-7.2_{-4.7}^{+4.5}$&$-7.5_{-4.5}^{+4.6}$&$-7.9_{-4.4}^{+4.7}$\\ 

$L(\mathrm{H_2O})$&-3.000&$-2.9_{-0.7}^{+0.8}$&$-2.4_{-0.8}^{+0.9}$&$-2.8_{-0.8}^{+0.8}$&$-2.8_{-0.8}^{+0.7}$&$-2.8_{-0.9}^{+0.9}$&$-2.4_{-0.9}^{+0.9}$&$-2.7_{-0.7}^{+0.6}$&$-2.8_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CO_2})$&-3.387&$-4.3_{-1.9}^{+1.1}$&$-3.3_{-0.8}^{+0.8}$&$-3.4_{-0.7}^{+0.7}$&$-3.3_{-0.7}^{+0.7}$&$-3.7_{-0.8}^{+0.9}$&$-3.0_{-0.8}^{+0.8}$&$-3.1_{-0.6}^{+0.6}$&$-3.2_{-0.6}^{+0.6}$\\ 

$L(\mathrm{CH_4})$&-5.770&$-10.0_{-2.9}^{+3.1}$&$-8.7_{-3.9}^{+2.9}$&$-6.5_{-3.7}^{+1.0}$&$-5.9_{-0.9}^{+0.8}$&$-8.6_{-3.7}^{+2.6}$&$-5.8_{-1.6}^{+1.0}$&$-5.6_{-0.7}^{+0.6}$&$-5.6_{-0.6}^{+0.6}$\\ 

$L(\mathrm{O_3})$&-6.523&$-6.8_{-0.6}^{+0.6}$&$-6.3_{-0.6}^{+0.6}$&$-6.5_{-0.5}^{+0.5}$&$-6.5_{-0.6}^{+0.6}$&$-6.6_{-0.6}^{+0.6}$&$-6.2_{-0.6}^{+0.7}$&$-6.3_{-0.5}^{+0.5}$&$-6.4_{-0.4}^{+0.4}$\\ 

$L(\mathrm{CO})$&-6.903&$-7.1_{-4.5}^{+4.3}$&$-7.4_{-4.4}^{+4.6}$&$-7.5_{-4.7}^{+4.7}$&$-7.4_{-4.6}^{+4.5}$&$-7.4_{-4.6}^{+4.4}$&$-7.7_{-4.5}^{+4.8}$&$-7.1_{-4.7}^{+4.3}$&$-7.6_{-4.6}^{+4.7}$\\ 

$L(\mathrm{N_2O})$&-6.495&$-8.8_{-3.7}^{+3.6}$&$-8.4_{-3.8}^{+3.5}$&$-9.2_{-3.4}^{+3.4}$&$-9.4_{-3.5}^{+3.2}$&$-8.7_{-3.7}^{+3.8}$&$-8.8_{-3.7}^{+3.5}$&$-9.2_{-3.6}^{+3.3}$&$-9.6_{-3.3}^{+3.3}$\\
\hline
\end{tabular}
\tablefoot{Here, $L(\cdot)$ stands for $\log_{10}(\cdot)$.}
\end{table*}

\egroup
